Overlap-guided Gaussian Mixture Models for Point Cloud Registration

Probabilistic 3D point cloud registration methods have shown competitive performance in overcoming noise, outliers, and density variations. However, registering point cloud pairs in the case of partial overlap is still a challenge. This paper proposes a novel overlap-guided probabilistic registration approach that computes the optimal transformation from matched Gaussian Mixture Model (GMM) parameters. We reformulate the registration problem as the problem of aligning two Gaussian mixtures such that a statistical discrepancy measure between the two corresponding mixtures is minimized. We introduce a Transformer-based detection module to detect overlapping regions, and represent the input point clouds using GMMs by guiding their alignment through overlap scores computed by this detection module. Experiments show that our method achieves superior registration accuracy and efficiency than state-of-the-art methods when handling point clouds with partial overlap and different densities on synthetic and real-world datasets. https://github.com/gfmei/ogmm

==> sections/exp_backup.tex <==
\section{Methods}
\begin{figure*}[t]
	\centering
	\includegraphics[width=1.0\textwidth]{figures/main_chart.pdf}
	\vspace{-.3cm}
	\caption{The architecture of our \ourmethod consists of three modules: feature extraction, overlap region detection, and overlap-guided GMM for registration.
	\fabiocomment{This figure requires a more detailed caption.}
	}
	\label{fig:gmm}
\end{figure*}

Rigid point cloud registration refers to recover a rigid transformation matrix $T\in SE(3)$, \gmei{which consists of rotation $R\in SO(3)$ and translation $\bm{t}\in \mathbb{R}^3,$} that optimally aligns the source point cloud $\bm{\mathcal{P}}=\{\bm{p}_i \in\mathbb{R}^{3}\big|i = 1, 2, ..., N\}$ to the target point cloud $\bm{\mathcal{Q}}=\{\bm{q}_j \in\mathbb{R}^{3}\big|j = 1, 2, ..., M\}$, where N and $M$ represent the number of points in $\bm{\mathcal{P}}$ and $\bm{\mathcal{Q}}$, respectively. 
Fig.~\ref{fig:gmm} illustrates our framework that consists of three modules: feature extraction, overlap region detection, and overlap-guided GMM for registration. 
The shared weighted encoder extracts point-wise features $\bm{\mathcal{F}}_p$ and $\bm{\mathcal{F}}_q$ from point clouds $\bm{\mathcal{P}}$ and $\bm{\mathcal{Q}}$, respectively.
The self-attention module is used to update the point-wise features $\bm{\mathcal{F}}_p$ and $\bm{\mathcal{F}}_q$, which are context-aware. 
The overlap region detection module projects the updated features $\bm{\mathcal{P}}$ and $\bm{\mathcal{Q}}$ to overlap scores $\bm{o}_p, \bm{o}_q$, respectively.  
$\bm{\mathcal{F}}_p$, $\bm{\mathcal{F}}_q$, $\bm{o}_p$ and $\bm{o}_q$ are used to estimate the distributions (GMM) of $\bm{\mathcal{P}}$ and $\bm{\mathcal{Q}}$. 
Weighted SVD is used to estimate the rigid transformation $T$ based on the estimated distributions.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Feature Extraction}

% {\color{red}
The feature extraction network consists of a Dynamic Graph Convolutional Neural Network (DGCNN), positional encoding and a clustered self-attention network. 
% Next, we will introduce them in detail.}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \subsubsection{Encoder.}
Given a point cloud pair $\bm{\mathcal{P}}$ and $\bm{\mathcal{Q}}$, we apply DGCNN as an encoder to extract the associated features $\bm{\mathcal{F}}_{p}=\{\bm{f}_{p_i} \in\mathbb{R}^{3}\big|i = 1, 2, ..., N\}$ and $\bm{\mathcal{F}}_{q}=\{\bm{f}_{q_j} \in\mathbb{R}^{3}\big|j = 1, 2, ..., M\}$. 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Attention module}
% Transformers have become one of the dominant architectures in deep learning,
% particularly as a powerful alternative to convolutional neural networks (CNNs) in computer vision. 
% However, 
Transformer training and inference in previous works can be prohibitively expensive due to the quadratic complexity of self-attention over a long sequence of representations, especially for high-resolution correspondences prediction tasks. 
To mitigate this limitation, our novel clustering-based Transformer architecture operates after local feature extraction:
$\bm{\mathcal{F}}_p$ and $\bm{\mathcal{F}}_q$ are passed through the attention module to extract context dependent point-wise features. 
Intuitively, the self-attention module transforms the DGCNN features into more informative representations to facilitate matching.

\vspace{.1cm}
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\noindent \textbf{Spherical positional encoding.}
Transformers are typically fed with only high-level features, which may not explicitly encode the geometric structure of the point cloud~\cite{wang2019deep,huang2021predator}.
This makes the learned features geometrically less discriminative, causing severe matching ambiguity and numerous outlier matches, especially in low-overlap cases~\cite{qin2022geometric}.
A straightforward recipe is to explicitly inject positional encoding of 3D point coordinates, which assigns intrinsic geometric properties to the per-point feature by adding unique positional information that enhances distinctions among point features in indistinctive regions \cite{zhao2021point}. 
However, the resulting coordinate-based attentions are naturally transformation-variant \cite{qin2022geometric}, while registration requires transformation invariance since the input point clouds can be in arbitrary poses. 
To this end, we design spherical positional encoding, which leverages the distances and angles computed with the points, to encode the transformation-invariant geometric information of the points. 
Specifically, given a point $\bm{p}_i \in \bm{\mathcal{P}}$, we select the $k>0$ nearest neighbors $\mathcal{K}_i$ of $\bm{p}_i$ and compute the centroid $\bm{p}_c=\sum_{i=1}^{N}\bm{p}_i$ of mass of $\bm{\mathcal{P}}$. 
For each $\bm{p}_x\in \mathcal{K}_i$, we denote the angle between the vectors $\bm{p}_i-\bm{p}_c $ and $ \bm{p}_x-\bm{p}_c$ as $\alpha_{ix}$. 
The positional encoding $\bm{f}^{pos}_{p_i}$ of $\bm{p}_i$ is defined as 
%+++++++++++++++++++++++++++++++++++++++++++++
\begin{equation}\label{eq:pos}
	\bm{f}^{pos}_{p_i} = \varphi\left(\|\bm{p}_i-\bm{p}_c\|_2\right) +\max_{x\in \mathcal{K}_i}\{\phi\left(\alpha_{ix}\right)\},
\end{equation}
%+++++++++++++++++++++++++++++++++++++++++++++
where $\varphi$ and $\phi$ are two MLPs, and each MLP consists of a linear layer and one ReLU nonlinearity function.
Our positional encoding is invariant to rigid transformation since the distance and angles are invariant to transformation.


\vspace{.1cm}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\noindent \textbf{Cluster-based self-attention.}
The extracted local features have a limited receptive field which may hinder distinctiveness of regions. 
Instead, humans can find correspondences between these regions not only based on the local neighborhood structures but also by exploiting context.
Self-attention is thus introduced to model global structures by establishing long-range dependencies.
We exploit this idea to improve the computational complexity of self-attention.
Specifically, we first use K-Means to cluster point cloud $\bm{\mathcal{P}}$ (or $\bm{\mathcal{Q}}$) into $J$ non-overlapping clusters in geometric space by $\bm{\gamma}^p\in \{0, 1\}^{N\times J}$ such that, $\gamma^p_{ij}=1$ (or $\gamma^q_{ij}=1$), if the $i$-th point of $\bm{\mathcal{P}}$ (or $\bm{\mathcal{Q}}$) belongs to the $j$-th cluster (denoted as $\bar{\bm{p}}_j$ or $\bar{\bm{q}}_j$) and 0 otherwise. Using this partitioning, we can now compute the clustered attention. Let $\bm{\mathcal{F}}^l_{\bm{p}}$ be the intermediate representation for $\bm{\mathcal{P}}$ at layer $l$ and let $\bm{\mathcal{F}}^0_{\bm{p}}=\{\bm{f}^{pos}_{\bm{p}_i}+\bm{f}_{\bm{p}_i}\}$. 
First, we can calculate the cluster centroids $\bm{f}_{\bar{p}_j}$ and $\bm{f}_{\bar{q}_j}$ of the points in each of these $J$ clusters in feature space as follows,
%+++++++++++++++++++++++++++++++++++++++++++++
\begin{equation}\label{eq:fcentroids}
    \begin{aligned}
    \bm{f}_{\bar{p}_j} &= \frac{1}{\sum_i^N\gamma^p_{ij}}\sum_{i=1}^N\gamma^p_{ij}\bm{f}_{p_i}, \\
    \bm{f}_{\bar{q}_j} &= \frac{1}{\sum_j^M\gamma^q_{ij}}\sum_{i=1}^M\gamma^q_{ij}\bm{f}_{q_j}.
    \end{aligned}
\end{equation}
%+++++++++++++++++++++++++++++++++++++++++++++
We use a multi-attention layer with four parallel attention heads~\cite{wang2019deep}. 
The attention module updates $\bm{\mathcal{F}}^l_{\bm{p}}$ in parallel via
%+++++++++++++++++++++++++++++++++++++++++++++
\begin{equation}
    \bm{f}_{\bm{p}_i} \leftarrow \bm{f}_{\bm{p}_i} + \mbox{MLP}\left(\sum_{j=1}^J\alpha^{\bm{p}}_{ij}W^s_V\bm{f}_{\bar{\bm{p}}_j}\right),
\end{equation}
%+++++++++++++++++++++++++++++++++++++++++++++
where $\alpha^{\bm{p}}_{ij}$ is the element of matrix $\bm{\alpha}^{\bm{p}}=\mbox{Softmax}(\bm{S})$ with $\bm{S}=(W^s_Q\bm{f}_{\bm{p}_i})^\top W^s_K\bm{f}_{\bar{\bm{p}}_j}$. Here, $W^s_Q\in \mathbb{R}^{N\times d}, W^s_K\in \mathbb{R}^{J\times d}$ and $W^s_V\in \mathbb{R}^{J\times d}$ are the query, key and value matrices. The self-attention features for $\bm{\mathcal{Q}}$ are updated in the same
way. $\mbox{MLP}(\cdot)$ denotes a three-layer fully connected network with instance normalization \cite{ulyanov2016instance} and ReLU~\cite{xu2015empirical} activations after the first two layers.




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Overlap Region Detection}

\noindent\textbf{Cluster-based cross-attention.}
Cross-attention is a typical module for point cloud registration tasks, which performs feature exchange between two input point clouds. 
Given the self-attention feature matrices $\bm{\mathcal{F}}_{\bm{p}}$ and $\bm{\mathcal{F}}_{\bm{q}}$ for $\bm{\mathcal{P}}$ and $\bm{\mathcal{Q}}$ respectively, we update the cluster centroids $\bm{f}_{\bar{p}_j}$ and $\bm{f}_{\bar{q}_j}$ based on Eq.~\eqref{eq:fcentroids}. We denote the transformed features as $\bm{\mathcal{F}}^t_{p}$ and $\bm{\mathcal{F}}^t_{p}$ by cross-attention feature matrix via
%+++++++++++++++++++++++++++++++++++++++++++++
\begin{equation}
    \bm{f}^t_{\bm{p}_i} \leftarrow \bm{f}_{\bm{p}_i} + \mbox{MLP}\left(\sum_{j=1}^J\beta^{\bm{p}}_{ij}W^c_V\bm{f}_{\bar{\bm{q}}_j}\right),
\end{equation}
%+++++++++++++++++++++++++++++++++++++++++++++
where $\beta^{\bm{p}}_{ij}$ is the element of matrix $\bm{\beta}^{\bm{p}}=\mbox{SoftMax}(\bm{C})$ with $\bm{C}=(W^c_Q\bm{f}_{\bm{p}_i})^\top W^c_K\bm{f}_{\bar{\bm{q}}_j}$. Here, $W^c_Q\in \mathbb{R}^{N\times d}, W^c_K\in \mathbb{R}^{J\times d}$ and $W^c_V\in \mathbb{R}^{J\times d}$ are the query, key and value matrices.  $\mbox{MLP}(\cdot)$ denotes a three-layer fully connected network with instance normalization \cite{ulyanov2016instance} and ReLU~\cite{xu2015empirical} activations after the first two layers. The same cross-attention block is also applied in reverse direction, so that information flows in both directions, $\bm{\mathcal{P}}\rightarrow \bm{\mathcal{Q}}$ and $\bm{\mathcal{Q}}\rightarrow \bm{\mathcal{P}}$.

\vspace{.1cm}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\noindent\textbf{Overlap score prediction.}
To deal with non-overlapping points, an overlap score prediction block is proposed. 
After obtaining the conditioned features $\bm{\mathcal{F}}_p$ and $\bm{\mathcal{F}}_q$, the per-point overlap score $\bm{o}_{{p}_i} \in [0, 1]$ can be computed by
%+++++++++++++++++++++++++++++++++++++++++++++
\begin{equation}\label{eq:opcom}
	\begin{aligned}
		& w_{ij} = \text{Softmax}\left(\frac{1}{t}\left<\bm{f}^t_{p_i}, \bm{f}^t_{q_j}\right>\right), \\
		& \bm{o}_{p_i} = g_\beta\left(\mbox{cat}\left[\bm{f}^t_{q_i}, \bm{w}^{\top}_i g_\alpha \left(\bm{\mathcal{F}}^t_{q}\right)\right]\right),	
	\end{aligned}
\end{equation}
%+++++++++++++++++++++++++++++++++++++++++++++
where $\left<\cdot, \cdot\right> $ is the inner product, and $ t=0.1$ is the temperature parameter that controls the soft assignment. When $t\rightarrow 0$, $w_{ij}$ converges to a hard nearest-neighbor assignment. $g_\alpha\left(\cdot\right): \mathbb{R}^b\rightarrow [0, 1]$ and $g_\beta\left(\cdot\right): \mathbb{R}^{b+1}\rightarrow [0, 1]$ are linear layers followed by an instance normalization layer and a sigmoid activation with different parameters $\alpha$ and $\beta$, respectively.



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Overlap-guided GMM for Registration}
The core idea of \ourmethod is to represent discrete point clouds by Gaussian mixture models (GMM). A GMM establishes a multimodal generative probability distribution over 3D space as a weighted sum of $J$ Gaussian densities~\cite{yuan2020deepgmr}, with the form
%+++++++++++++++++++++++++++++++++++++++++++++
\begin{equation}\label{eq:density}
p(\bm{x})=\sum^J_{j=1}\pi_j\mathcal{N}\left(\bm{x}|\bm{\mu}_j,\bm{\Sigma}_j\right),\bm{x}\in \mathbb{R}^3.
\end{equation}
%+++++++++++++++++++++++++++++++++++++++++++++
Each Gaussian density $\mathcal{N}\left(\bm{x}|\bm{\mu}_j,\bm{\Sigma}_j\right)$ is referred to as a component of the GMM and parameterized by a mean $\bm{\mu}_j$ and covariance $\bm{\Sigma}_j$. The components are combined through a set of normalized mixing coefficients $\{\pi_1,\pi_2,\cdots,\pi_J\}$ that represent the prior probability of selecting the $j$-th component.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Learning Posterior}
We first apply a segmentation head $\phi_\alpha$ that takes as input $\bm{\mathcal{F}}_p$ and $\bm{\mathcal{F}}_q$ and outputs joint log probabilities, and a softmax operator that acts on log probabilities to generate a probability matrix $\bm{S}^p$ and $\bm{S}^q$, respectively. 

The GMM parameters $\bm{\Theta}_p$ for point cloud $\bm{\mathcal{P}}$ consists of $L$ triples $(\pi^p_{j},\bm{\mu}^p_{j},\bm{\Sigma}^p_{j})$, where $\pi^p_{j}$ is a scalar mixture weight, $\bm{\mu}^p_{j}$ is a $3\times 1$ mean vector and $\bm{\Sigma}^p_{j}$ is a $3\times 3$ covariance matrix of the $j$-th component. 
For partial overlapping registration tasks, given the outputs $\bm{S}^p$ of $\phi_\alpha$ together with the point coordinates $\bm{\mathcal{P}}$, and overlap scores $\bm{o}_p$, the GMM parameters can be written as
%+++++++++++++++++++++++++++++++++++++++++++++
\begin{equation}\label{eq:gmm}
    \begin{aligned}
    \pi^p_{j} &= \frac{1}{\sum_{i=1}^N\bm{o}_{p_i}}\sum_{i=1}^N\bm{o}_{p_i}\bm{s}^p_{ij}, \\
    n_p &= \pi^p_{j}\sum_{i=1}^N\bm{o}_{p_i} \quad \bm{\mu}^p_{j} = \frac{1}{\epsilon+n_p}\sum_{i=1}^N\bm{o}_{p_i}\bm{s}^p_{ij}\bm{p}_i,\\
    \bm{\Sigma}^p_{j} &= \frac{1}{\epsilon+n_p\pi^p_{j}}\sum_{i=1}^N\bm{o}_{p_i}\bm{s}^p_{ij}\left(\bm{p}_i-\bm{\mu}^p_{j}\right)\left(\bm{p}_i-\bm{\mu}^p_{j}\right)^\top,
    \end{aligned}
\end{equation}
%+++++++++++++++++++++++++++++++++++++++++++++
where $\epsilon=1e-4$ is used to avoid zero in the denominator. By the same way, we can get the $\pi^q_{j}, \bm{\mu}^q_{j}$ and $\bm{\Sigma}^q_{j}$ for target point cloud, when giving $\bm{S}^q,\bm{o}_q$ and $\bm{\mathcal{Q}}$. The GMMs of point set $\bm{\mathcal{P}}$ and $\bm{\mathcal{Q}}$ are given as
%+++++++++++++++++++++++++++++++++++++++++++++
\begin{equation} \label{eq:post}
\begin{aligned}
    \mathbf{G}_{\mathcal{P}}\left(\bm{x}\right) &= \sum _{j=1}^{L}\pi^p_{j}\mathcal{N} \left(\bm{x}|\bm{\mu}^p_{j}, \bm{\Sigma}^p_{j}\right), \\
    \mathbf {G}_{\mathcal{Q}}\left(\bm{x}\right) &= \sum _{j=1}^{L}\pi^q_{j}\mathcal{N} \left(\bm{x}|\bm{\mu}^q_{j}, \bm{\Sigma}^q_{j}\right).
\end{aligned}
\end{equation}
%+++++++++++++++++++++++++++++++++++++++++++++


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Estimating the transformation.}
Given the estimated GMMs parameters estimated through Eq.~\eqref{eq:post}, we obtain the optimal transformation $T$ in a closed-form solution by minimizing the L2 between two Gaussian mixtures as
%+++++++++++++++++++++++++++++++++++++++++++++
\begin{equation*}\label{eq:l2dis}
d_{L2}\left (\mathbf{G}_{\mathcal{P}}, \mathbf{G}_{\mathcal{Q}}\left(\bm{x}\right), T\right) = \int \left (\mathbf{G}_{\mathcal{P}}\left(\bm{x}\right)-T\left(\mathbf{G}_{\mathcal{Q}}\right)\right)^{2}d\bm{x}. 
\end{equation*}
%+++++++++++++++++++++++++++++++++++++++++++++
The closed-form expression of the L2 distance between two Gaussian mixtures can be easily derived using the following formula \cite{jian2010robust}:

%+++++++++++++++++++++++++++++++++++++++++++++
\begin{equation*} 
\int\mathcal{N}\left(\bm{x}|\bm{\mu}_i,\bm{\Sigma}_i\right)\mathcal{N}\left(\bm{x}|\bm{\mu}_j,\bm{\Sigma}_j\right) = \left ({0|\bm{\mu}_i - \bm{\mu}_j, \bm{\Sigma}_i + \bm{\Sigma}_j}\right).
\end{equation*}
%+++++++++++++++++++++++++++++++++++++++++++++
For rigid point cloud registration, $\int \left (T\left(\mathbf{G}_{\mathcal{Q}}\right)\left(\bm{x}\right)\right)^{2}d\bm{x}=\int \left (\mathbf{G}_{\mathcal{Q}}\left(\bm{x}\right)\right)^{2}d\bm{x}$, i.e., itremains invariant under rigid transformation. Thus, it can be approxiated by
%+++++++++++++++++++++++++++++++++++++++++++++
\begin{equation}\label{eq:wsvd}
   \min_{T}\sum_{j=1}^J\frac{\pi^p_j+\pi^q_j}{\sigma^p_j+\sigma^q_j}\|T(\bm{\mu^p_j})-\bm{\mu^p_j})\|,
\end{equation}
%+++++++++++++++++++++++++++++++++++++++++++++
where $\sigma^k_j$represents the spectral norm of matrix $\bm{\Sigma}k_j$ with $k=p,q$. We can solve $T$ in closed form using a weighted version of the SVD solution~\cite{yuan2020deepgmr}.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Training}\label{sec:training}
We simultaneously predict overlapping regions, cluster point clouds, and estimate rigid transformations, so that three loss functions are proposed to supervise the above two procedures separately.

\vspace{.1cm}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\noindent\textbf{Global registration loss.}\label{subs:clus}
We first exploit the registration error based loss function to train our model. To handle the partially-overlapping problem well, we adopt a robust error metric that does not incur high computational overhead. Specifically, we formulate the registration loss as
%+++++++++++++++++++++++++++++++++++++++++++++
\begin{equation}
\begin{aligned}
    \mathcal{L}_g\left(\bm{\mathcal{\bar{P}}}, \bm{\mathcal{Q}}\right) &=\sum_{\bar{\bm{p}}\in\bm{\mathcal{\bar{P}}}}\psi_{\nu}\left(\min_{\bm{q}\in\bm{\mathcal{Q}}}\|\bar{\bm{p}}-\bm{q}\|_2^2\right) \\
    & +\sum_{\bm{q}\in\bm{\mathcal{Q}}}\psi_{\nu}\left(\min_{\bar{\bm{p}}\in\bm{\mathcal{\bar{P}}}}\|\bar{\bm{p}}-\bm{q}\|_2^2\right),
\end{aligned}
\end{equation}
%+++++++++++++++++++++++++++++++++++++++++++++
where $\bm{\mathcal{\bar{P}}}$ denotes the transformed source point cloud with the estimated transformation. $\psi_{\nu}$ is the Welsch’s function~\cite{holland1977robust}:
%+++++++++++++++++++++++++++++++++++++++++++++
\begin{equation}
    \psi_{\nu}\left(x\right)=1-\exp\left(-\frac{x^2}{2\nu^2}\right),
\end{equation}
%+++++++++++++++++++++++++++++++++++++++++++++
and $\nu > 0$ is a user-specified parameter.

\vspace{.1cm}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\noindent\textbf{Clustering-based loss.}
To ensure that our network learns a consistent GMM representation across feature and geometric space rather than fit a GMM in a single feature space. We introduce the following loss.
%+++++++++++++++++++++++++++++++++++++++++++++
\begin{equation}
\begin{aligned}
    \mathcal{L}_{c} = &-\sum_{ij}\gamma^p_{ij}\log \frac{\exp{\left(-\|\bm{p}_i-\bm{\mu^p_j}\|^2_2\right)}}{\sum_l\exp{\left(-\|\bm{p}_i-\bm{\mu^p_l}\|^2_2\right)}} \\
    & -\sum_{ij}\gamma^q_{ij}\log \frac{\exp{\left(-\|\bm{q}_i-\bm{\mu^q_j}\|^2_2\right)}}{\sum_l\exp{\left(-\|\bm{q}_i-\bm{\mu^q_l}\|^2_2\right)}}.
\end{aligned}
\end{equation}
%+++++++++++++++++++++++++++++++++++++++++++++


\vspace{.1cm}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\noindent\textbf{Overlap score loss.} 
The goal of the overlap score loss is to segment the overlap region between $\bm{\mathcal{P}}$ and $\bm{\mathcal{Q}}$. 
The ground-truth label $\bar{\bm{o}}_{p_i}$ of point $\bm{p}_i$ is defined as
\begin{equation}\label{eq:gtop}
	\bar{\bm{o}}_{p_i} = 
	\begin{cases}
		1, & \left(\min_{q_j\in \bm{\mathcal{Q}}}\|\bar{\bm{T}}(\bm{p}_i) -\bm{q}_j\|\right) < \eta \\
		0, & \text{otherwise}
	\end{cases},
\end{equation}
$\bar{\bm{o}}_{q_j}$ is calculated in the same way. 
The overlap score loss is defined as $\mathcal{L}_{O} = \frac{1}{2}\left(\mathcal{L}_{\bm{\mathcal{P}}} + \mathcal{L}_{\bm{\mathcal{Q}}} \right)$, where
%+++++++++++++++++++++++++++++++++++++++++++++
\begin{equation*}
	\mathcal{L}_{\bm{\mathcal{P}}} = \frac{-1}{|\bm{\mathcal{P}}|}\sum_{i}\left(\bar{\bm{o}}_{\bm{p}_i}\log \bm{o}_{\bm{p}_i}+\left(1-\bar{\bm{o}}_{\bm{p}_i}\right)\log\left(1-\bm{o}_{\bm{p}_i}\right)\right)
\end{equation*}
%+++++++++++++++++++++++++++++++++++++++++++++
By the same operation,  we can attain $\mathcal{L}_{\bm{\mathcal{Q}}}$. 
